Distillation Enhanced Time Series Forecasting Network with Momentum Contrastive Learning

Contrastive representation learning is crucial in time series analysis as it alleviates the issue of data noise and incompleteness as well as sparsity of supervision signal. However, existing constrastive learning frameworks usually focus on intral-temporal features, which fails to fully exploit the intricate nature of time series data. To address this issue, we propose DE-TSMCL, an innovative distillation enhanced framework for long sequence time series forecasting. Specifically, we design a learnable data augmentation mechanism which adaptively learns whether to mask a timestamp to obtain optimized sub-sequences. Then, we propose a contrastive learning task with momentum update to explore inter-sample and intra-temporal correlations of time series to learn the underlying structure feature on the unlabeled time series. Meanwhile, we design a supervised task to learn more robust representations and facilitate the contrastive learning process. Finally, we jointly optimize the above two tasks. By developing model loss from multiple tasks, we can learn effective representations for downstream forecasting task. Extensive experiments, in comparison with state-of-the-arts, well demonstrate the effectiveness of DE-TSMCL, where the maximum improvement can reach to 27.3%.

==> response/response_letter.tex <==
Response Letter
1 Detailed response to Reviewer #1
Thank you very much, Reviewer #1, for your thorough and professional feedback. I deeply value your comments and suggestions, which have been instrumental in refining our work. We have carefully considered each point and have made every effort to address each of them accordingly.
Comment 1: [Clear Domain Contribution] The authors failed to explain the innovations and contributions of the manuscript. What are the improvements/innovations of the proposed method? How to solve these problems? The manuscript's innovations are not significant.
Answer: 

Comment 2: [Time Series Characteristics] What are the characteristics of time series data? What are the challenges of time series analysis and forecasting? The relevant time series literature is missing in the manuscript, e.g., "Densely Knowledge-Aware Network for Multivariate Time Series Classification" (TSMC). Meanwhile, this literature can help the authors solve the problems above.
Answer: 
                           %↑(TSMC)
% 59. Zhiwen Xiao, ！！!!!Huanlai Xing*!!!！！, Rong Qu, Li Feng, Shouxi Luo, Penglin Dai, Bowen Zhao, and Yuanshun Dai. Densely Knowledge-aware Network for Multivariate Time Series Classification.  IEEE Transactions on Systems, Man, and Cybernetics: Systems, Early Access, 2023. DOI: 10.1109/TSMC.2023.3342640 (SCI一区)
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{TSMC.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

Comment 3: [Research Gaps] There are some similar contrastive learning methods in time series, e.g., "Deep Contrastive Representation Learning With Self-Distillation" (TETCI) and "CapMatch: Semi-Supervised Contrastive Transformer Capsule With Feature-Based Knowledge Distillation for Human Activity Recognition" (TNNLS). The authors must clearly explain the difference(s) between the proposed method and similar works in the introduction. The authors should further highlight the manuscript's innovations and contributions in the manuscript.
Answer: 
     %                  ↑ (TETCI)
% 58. Zhiwen Xiao, ！！!!!Huanlai Xing!!!！！*, Bowen Zhao, Rong Qu, Shouxi Luo, Penglin Dai, Ke Li, and Zonghai Zhu. Deep Contrastive Representation Learning With Self-Distillation. IEEE Transactions on Emerging Topics in Computational Intelligence, Early Access, 2023. DOI: 10.1109/TETCI.2023.3304948 (SCI二区)
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{reviewer1-Q3-1.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

 %                      ↑(TNNLS)
%60. Zhiwen Xiao, Huaguang Tong, Rong Qu, ！！!!!Huanlai Xing!!!！！*, Shouxi Luo, Zonghai Zhu, Fuhong Song, and Li Feng. CapMatch: Semi-supervised Contrastive Transformer Capsule with Feature-based Knowledge Distillation for Human Activity Recognition. IEEE Transactions on Neural Networks and Learning Systems, Early Access, 2023. DOI: 10.1109/TNNLS.2023.3344294 (SCI一区)   

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{response/image.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

%这三篇文章在arxiv检索不到

Comment 4: [Reasoning] The authors should provide some necessary mathematical reasonings.
Answer: 

Comment 5: [Computational complexity] Computational complexity should be analyzed and compared in the manuscript.
Answer: We apologize for the oversight in not providing an analysis and comparison of computational complexity in our initial submission. We are deeply grateful for your insightful comments, which have prompted us to address this gap in our revised draft.
To rectify this, we have included a table that compares our model with the baseline model in terms of computational complexity. The revised version now includes the following description below the table to provide context and clarity:

Table 3 shows the runtime in seconds for each phase of different representation learning methods and end-to-end approaches. All DE-TSMCL experiments were performed on an NVIDIA GeForce GTX 1060(6G) GPU. Note that for Informer, we follow the hyperparameters (including lookback window length) as described by the authors, which may vary for different forecast horizons. Consequently, the runtime may not strictly increase with the forecast horizon. We would like to emphasize that the ridge regressor fractions should be equivalent for all representation learning approaches, since the dimension size used is the same for all methods, and any differences are only due to randomness. Despite a slightly longer training time compared to some baseline approaches, DE-TSMCL gives much better results.
Table 3 shows that the training time for DE-TSMCL is relatively short. This is because our projection layer is based on a simple MLP and the encoder's choice of a simple convolutional framework. This approach is well suited for time series tasks, as it allows for the extraction of sequence features without requiring overly complex architectures.
However, it is unfortunate that DE-TSMCL has a relatively long inference time. This is a consequence of our joint optimization strategy, which introduces more computational complexity than previous models. Nevertheless, the strategy provides a significant performance improvement that compensates for the inference time penalty during the training phase. Of course, this could also be due to the older nature of our device (NVIDIA GeForce GTX 1060(6G) GPU). Overall, our model is comparable to the state-of-the-art in terms of time complexity. However, our model provides superior performance with a simpler architecture, which facilitates future research and extensions. We hope that these additions will satisfy your request and provide a more comprehensive view of our model’s computational efficiency.
Thank you once again for your important feedback, which has significantly improved the quality of our work.

Comment 6: [Limitations] Could you tell me the limitations of the proposed method? How will you solve them? Please add this part to the manuscript.
Answer: We understand the concerns of the reviewer considering limitation of the study. Now limitation of the study was incorporated in the article. It is clear that our study has limitation. 
We write the limitations of this paper as well as future solutions in Conclusion:
In this paper, we introduce a Distillation Enhanced Time Series Network with Momentum Contrastive Learning (DE-TSMCL).   Within the DE-TSMCL framework, we incorporate knowledge distillation between models that use overlapping sub-series to represent time series data for forecasting tasks.   We further integrate the benefits of two types of tasks to improve the expressiveness of the model. 
We conduct extensive experiments on four real-world datasets, and the results show that DE-TSMCL outperforms other state-of-the-art models in various scenarios.   On the ETTm1 dataset, which contains a considerable amount of data, {DE-TSMCL} achieves a 24.2\% improvement in MSE and a 14.7\% improvement in MAE.  On the ETTh1 dataset, {DE-TSMCL} also achieves similar gains (14.2\% improvement in MSE and 10.6\% in MAE). 
However, we also find the limitations of the proposed method. Although we include an additional supervised loss to address the challenges of momentum updating for small datasets and short lookback windows, the performance improvements of DE-TSMCL on small datasets are not as robust as those of previous methods.   We believe that the momentum update and additional supervised loss may indeed allow us to use the data multiple times for better prediction performance.   However, if the selected subsequence contains more outliers, this may have a more significant negative impact on representation learning.   Finally, repeated training with outliers may interfere with the model learning the trend and periodicity of the normal time series.   We speculate that the novel supervised loss may introduce conflicting objectives, optimizing for forecasting error under one set and representation learning under another, potentially destabilizing the training dynamics.   Furthermore, the new loss function design introduces additional hyperparameters, requiring a longer search for the optimal balance.   In essence, the current configuration may not be fully optimized.   In future work, we can explore adaptive hyperparameter search techniques, which have gained popularity in recent years, to replace our manual hyperparameter tuning for improved performance. 
Furthermore, as highlighted in the ablation study, the sensitivity of the model to parameter tuning requires more iterations and adjustments to consistently achieve optimal performance.   Therefore, identifying strategies to harmonize multiple modules and exploit their collective strengths is an important future research direction. 
In the future, we plan to investigate other convolutional techniques, including sparse convolutions in 3D point clouds and innovative CNN architectures, as well as experiment with more novel loss functions, such as rank-based cross-entropy loss and triplet loss, to further refine our forecasting capabilities. 
Last but not least, we maintain that the utility of established, albeit traditional, methods such as hierarchical convolutions, distillation frameworks, and contrastive learning paradigms has not been fully exploited in time series analysis. We earnestly anticipate that these established practices will continue to play a significant role in contemporary research.


Comment 7: [Typos] Please polish the manuscript carefully.
Answer: We sincerely apologize for the typos that marred the readability of our manuscript and potentially hindered your review process. We recognize that it is our responsibility to ensure the manuscript is meticulously polished to avoid such oversights.
The revised version now includes corrections to the typos in the conclusion and addresses the missing punctuation in the middle and end of sentences throughout other sections. We have strived to rectify any inaccuracies in our expressions to enhance your understanding of the manuscript.
In conclusion, we extend our deepest gratitude for your careful review and for identifying the typos and other expression errors within the manuscript. Your meticulous and serious approach is commendable and serves as an excellent example for all scientific research workers.


-----End of Response to Reviewer #1------


2 Detailed response to Reviewer #5
Thanks very much for your time to review this manuscript. We appreciate your elaborate efforts in reviewing. The new version takes into account your main comments. Please find my itemized responses in below and my revisions/corrections in the re-submitted files.
Reviewer detailed comments and our responses are as follows:
Comment 1: What is the meaning of the content marked in red after the output of the teacher network and student network in Figure 1?
Answer: We are sorry for not explaining the meaning of content marked in red. In the revised manuscript, we have supplemented the missing explanation in the end of Section 4.4 (The next paragraph of Eq.11.): Inspired by the drawings in DINO (Emerging Properties in Self-Supervised Vision Transformers) article, we apply the stop gradient (s-g) operator on the teacher to propagate the gradient (gradient) only through the student. The teacher parameters are updated with the exponential moving average (Ema) of the student parameters. Specifically, since red often signifies prohibition, we depict a red mark (s-g) following the teacher network in Figure 1 to signify the cessation of gradient updates. To achieve color uniformity among operators and the symmetry of the processes underlying the teacher-student network’s output, we append a gradient return marker of the same color to the student network, matching our pseudocode.

Comment 2: The model input is two randomly sampled sub-series with overlap. For long time series forecasting, do sampling location and overlap size affect model performance?
Answer: Thank you for your insightful comments. We appreciate your attention to detail and your understanding of the challenges associated with learning representations from randomly sampled series of varying sizes and locations.
In response to your observation, we agree that when the length of the sampled sequence is too short, the previous model may indeed struggle to learn effective representations. To address this issue, we have employed a momentum update mechanism. This approach allows for a slower update of the encoder parameters, which we have found to be beneficial in mitigating the impact of peak and trough data on the model’s performance. 
Furthermore, we have incorporated additional supervised tasks into our training regimen. By doing so, we are not only making use of the available data more efficiently but also ensuring that the representations learned are complementary to those provided by the teacher in the self-supervised task. As a result, our model exhibits greater robustness to variations in sampling location and sequence overlap size.
We acknowledge that our original description of these aspects in the manuscript lacked clarity and precision. We will take your feedback into account and enhance the relevant sections to provide a more thorough and coherent explanation.

Comment 3: Teacher network and student network share the same framework while using different parameters set. Please specify the difference.
Answer: First and foremost, we would like to express our gratitude for your careful review and for highlighting the need for a more detailed explanation of the momentum update mechanism in our manuscript. Your feedback is invaluable, and we are keen to address the concerns you have raised. 
You are correct in pointing out that the teacher and student networks share the same structure, as illustrated in Figure 2. To clarify the initialization process, we copy the parameters from the student network to the teacher network as an initial step (indicated by the first line of pseudo-code). During back-propagation, we update the student network’s parameters while halting the update for the teacher network’s parameters (denoted as s-g). This ensures that the teacher network retains a stable output. 
We have adopted the momentum update method, which is a common practice in computer vision image classification tasks. This method involves copying the student network’s parameters to the teacher network at a slower rate of 0.001, thus providing the teacher network with a stable output (as shown in Eq.11 and line 25 of the pseudocode). In Figure 1, we have used red markers to distinctly indicate the s-g operation and will reformulate this in Eq.11 in the revised draft for clarity. 
We acknowledge that our initial explanation of the momentum update was insufficient, and we apologize for any confusion this may have caused to readers less familiar with this operation. In the revised manuscript, we will dedicatedly expand on the explanation of the momentum update, ensuring that it is comprehensible to experts across the field without relying solely on references to related literature. 
Thank you once again for your constructive comments, which will undoubtedly enhance the quality and readability of our paper.

% for param_q, param_k in zip(
%             self.encoder_q.parameters(), self.encoder_k.parameters()
%         ):
%             param_k.data.copy_(param_q.data)  # initialize
%             param_k.requires_grad = False  # not update by gradient


 % def _momentum_update_key_encoder(self):
 %        """
 %        Momentum update of the key encoder
 %        """
 %        for param_q, param_k in zip(
 %            self.encoder_q.parameters(), self.encoder_k.parameters()
 %        ):
 %            param_k.data = param_k.data * self.m + param_q.data * (1.0 - self.m)

% momentum = 0.999
%                 for p_t, p_s in zip(self.teacher_net.parameters(), self.student_net.parameters()):
%                     p_t.data = momentum * p_t.data + (1. - momentum) * p_s.data 

% for p_t, p_s in zip(self.teacher_net.parameters(), self.student_net.parameters()):   
%   p_t.data = momentum * p_t.data + (1. - momentum) * p_s.data
Comment 4: Some details of the experiment may need further explanation. For example, what are the predicted horizon and overlapping subsequence length, respectively? How to implement univariate time prediction?
Answer: Thank you for your insightful comments. We appre


Comment 5: Please add an experiment in 5.6 based on the following settings: data augmentation is performed before the projection layer for the teacher network, while after the projection layer for the student network.
Answer: Thank you for your insightful comments. We appreciate your attention to detail and your understanding of the challenges associated with le

Comment 6: Symbols of the same meaning should be unified, and one symbol should not mean more than one meaning. For example, in 3.1 and 5.1.3, P and H represent the prediction horizon, respectively. P also has other meanings in Figure 2. In Table 1 and 5.1.4, T and l represent the length of look-back window, respectively.
Answer: We are deeply appreciative of the meticulous attention you have given to our manuscript, particularly regarding problem definition and notation use. Your feedback has been instrumental in improving the clarity of our work. 
Upon completing the manuscript, it became apparent that certain definitions had the potential to cause ambiguity. To address this, I decided to revise our symbols to avoid any confusion.   However, it seems that in doing so, I may have inadvertently introduced new ambiguities by assigning multiple meanings to certain symbols, which is indeed regrettable. 
We have carefully reviewed and corrected the errors you have highlighted in the revised version of our manuscript. For instance, we have unified the symbol H to represent the forecast horizon in Sections 3.1 and 5.1.3.
We have provided a brief re-introduction of the corresponding meaning of the symbol P in Figure 2 in the paragraph above Equation 5 in Section 4.3.1: To achieve a larger receptive field for each input, multiple causal convolution layers are usually stacked, so in this paper we use P as the maximum stacked convolution layers.
Furthermore, we have standardized the symbol T to represent the look-back window length in Table 1 and Section 5.1.4. 
We are truly grateful for your thorough and careful review, which has helped us to rectify errors that should not have been present in the manuscript. Your detailed corrections have significantly enhanced the quality and precision of our work.


Comment 7: There are still some mistakes that need to be corrected. For example, in 3.1, x∈T^(T×C); in Table1, Z∈R^(N×T×C); in 4.2.1, {a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}, b₁
Answer: We would like to express our sincere apologies for the various small errors that were present in our manuscript. We are deeply grateful for your careful review, which has helped us identify errors in the formatting of our mathematical symbols, as well as other issues with spelling, punctuation, and the correct marking of mathematical symbols.
In response to your comments, we have made the following corrections to the revised manuscript:
Changed “x∈T^(T×C)” in Section 3.1 to “x∈R^(T×C)”;
In Table 1, the set “Z∈R^(N×T×C)” was mentioned but not utilized in our paper. This set was initially intended to represent the outputs z generated after the MLP operation. However, upon your reminder, we agree that it is unnecessary to include this set in the manuscript. Therefore, we have deleted it from Table 1 to avoid any confusion caused by the presence of unused symbols;
In Section 4.2.1, the expression “{a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}” has been corrected to “{a₁,b₁,a₂,b₂,}∈{1,2,⋯,N}” in the revised version to accurately represent our intended notation.
We appreciate your rigorous, serious, and responsible attitude, and we find your suggestions to be very helpful. Your contributions have greatly improved the completeness and accuracy of our manuscript

We would like to reiterate our appreciation to Reviewer #5 for the helpful comments provided in the review. All the recommendations you proposed are greatly helpful for our manuscript, we have considered these comments carefully and tried our best to address every one of them.
-----End of Response to Reviewer #5------












3 Detailed response to Reviewer #7
We are deeply appreciative of Reviewer #7's insightful feedback.  Your comments have been instrumental in enhancing our manuscript.  We have meticulously addressed each point, aiming to address your concerns in the revised submission.  We sincerely hope that the new version will satisfactorily address your queries.
Reviewer detailed comments and our responses are as follows:
Comment 1: .In order to support reproduction of the results and follow-up works, I suggest the Authors to publish their implementation (source codes) in a software repository (e.g. github), as it may be difficult to re-implement the approach (despite the pseudocode provided in the manuscript).

Answer: We are truly appreciative of your constructive and forward-looking comments.  Open-sourcing our work is indeed the next step we intend to take. 
You have raised a valid point.  While we have provided pseudocode to illustrate the flow of our method, the saying goes that there are a thousand hamlets in a thousand eyes.  It may be challenging for some researchers, particularly those less familiar with computer vision image classification tasks or time series prediction tasks, to replicate our method.  To address this, we are committed to making our code publicly available on GitHub.  We have included a link to the software repository on GitHub at the end of the abstract in our manuscript to facilitate access and support all researchers in their follow-up work. 
In conclusion, we are immensely grateful for your excellent suggestions regarding our manuscript.  We agree that open sourcing is a practice that benefits the research community and should be encouraged among researchers. 
Thank you once again for your valuable input

Comment 2: .It would be interesting to see if the observed differences are statistically significant?
Answer：We are sorry for not explaining the experimental results clearly. Here we have carefully explained the results and look forward to your approval.

Comment 3: The Authors could perform additional experiments on time series from other domains (finance, medicine, etc.), or focus more on the "energy" domain.
Answer: We are sorry for not explaining the experimental results clearly. Here we have carefully explained the results and look forward to your approval.

Comment additionally: The manuscript needs careful proofreading: I found a few typos, e.g. "relay" instead of "rely" (in the "Conclusions"), "thatelectric" (Section 5.1.1), the dot is missing at the end of the first sentence of Section 4.1. Last but not least: if the Authors really want to use sparse convolution from the domain of 3D reconstruction in their future work, as they write in the Conclusions, they could have a look at this study: https://link.springer.com/chapter/10.1007/978-3-031-41456-5_12
Answer: Thank you very much for the problem. We appreciate your careful review and have taken note of the identified typos. We apologize for any confusion caused by these errors. In the revised version, we have thoroughly proofread the manuscript and made the necessary corrections. Specifically, we have addressed the following issues:

In the "Conclusion" section, we have corrected the typo from "relay" to "rely" to ensure the  meaning is conveyed accurately. In Section 5.1.1, we have rectified the typo "thatelectric" to the "that electric". We have added the missing dot at the end of the first sentence of Section 4.1 to ensure proper punctuation.

Thank you for your valuable comment and for providing us with the reference to a relevant study on sparse convolution. We appreciate your suggestion and will certainly consider it for our future work.

In the revised version of the manuscript, we have discussed the recommended reference [2] and the potential incorporation of sparse convolution techniques into our research, which can be found in the last paragraph of Section 4.3.1, Page 7. We are particularly interested in exploring the proposed sparsity-invariant convolution from [2], as it offers valuable insights that can aid us in addressing the challenge of forecasting irregularly sampled time series. By investigating and adapting these techniques, we aim to enhance the accuracy and effectiveness of our forecasting models in such scenarios.

Furthermore, we recognize the potential of applying sparse convolution in the specific domain of 3D reconstruction. While our current work focuses on time series forecasting, we believe that exploring the application of sparse convolution in 3D reconstruction can open up new possibilities and contribute to advancements in both fields.

We sincerely appreciate your suggestion and the thoughtful review of our manuscript. Your feedback has been invaluable in improving the quality and scope of our research. 

-----End of Response to Reviewer #7------

























Response Letter

1 Detailed response to Reviewer #1
Thank you very much, Reviewer #1, for providing us with such thorough and professional feedback. We truly appreciate your valuable comments and suggestions, as they have played a vital role in refining our work. Each point you raised has been carefully considered, and we have made every effort to address them accordingly.
Comment 1: [Clear Domain Contribution] The authors failed to explain the innovations and contributions of the manuscript. What are the improvements/innovations of the proposed method? How to solve these problems? The manuscript's innovations are not significant.
Answer: We appreciate your comments regarding the innovations and contributions of our manuscript. We apologize if we did not adequately highlight the improvements and innovations of our proposed method. Allow us to address your concerns and provide a clearer explanation:

Improvements/Innovations of the Proposed Method:

Distillation Enhanced Time Series Forecasting: Our method introduces a novel approach that leverages knowledge distillation techniques to improve time series forecasting. We employ a teacher-student framework, where the student network learns from the more knowledgeable teacher network, enabling the transfer of valuable knowledge and improving forecasting accuracy.
Overlapping Sub-series and Knowledge Distillation: We innovate by applying knowledge distillation techniques among models that rely on different overlapping sub-series within the time series. This approach allows us to capture diverse temporal patterns and enhance the model's ability to handle various aspects of the data.
Joint Optimization of Supervised and Self-Supervised Learning: We design both supervised and self-supervised learning tasks specifically for time series forecasting. By jointly optimizing these tasks, we enable the model to extract meaningful representations and capture complex temporal dependencies more effectively.
Addressing Noisy and Inconsistent Gradients: To overcome the challenges posed by noisy and inconsistent gradients during back-propagation, we introduce the use of momentum contrastive training. This technique updates the teacher and student networks at different scales, mitigating the impact of noise and ensuring more stable training.

The paper effectively addresses several challenges and problems in time series forecasting, including:

Data Noise and Distribution Shift: Our model addresses the challenge of data noise and distribution shift by leveraging knowledge distillation techniques and incorporating multiple overlapping sub-series in the forecasting process. This approach enables the model to learn robust representations that are less affected by noisy or shifted data points.
Dependence on Single Salient Feature: By jointly optimizing supervised and self-supervised learning tasks, our model becomes less dependent on a single salient feature. It captures multiple aspects of the time series, allowing for more comprehensive and accurate forecasting.
False Positive Focusing in Contrastive Learning: The use of momentum contrastive training in our approach helps mitigate false positive focusing, ensuring that the teacher and student networks update at different scales. This leads to improved model performance and reduces the impact of inconsistent gradients.

Furthermore, we have rewritten the contributions and “conclusion” section of the paper to better highlight the innovations and advancements of our proposed method. We believe that these revisions will provide a clearer understanding of the novel aspects introduced in our work and emphasize the significance of our contributions.

Comment 2: [Time Series Characteristics] What are the characteristics of time series data? What are the challenges of time series analysis and forecasting? The relevant time series literature is missing in the manuscript, e.g., "Densely Knowledge-Aware Network for Multivariate Time Series Classification" (TSMC). Meanwhile, this literature can help the authors solve the problems above.
Answer: Thank you for your affirmation for our work. We are trying to answer these comments and looking forward to your approval. 
1.Characteristics of Time Series Data:
Time series data possesses several distinct characteristics:
Temporal Dependence: Time series data exhibits a sequential correlation, where each observation is dependent on previous observations.
Trend: Time series data can exhibit long-term increasing or decreasing patterns.
Seasonality: Many time series exhibit recurring patterns at fixed intervals, such as daily, weekly, or yearly cycles.
Irregularity: Time series data can also have irregular fluctuations, making it challenging to identify underlying patterns.
Noise: Time series data can be affected by random fluctuations and measurement errors.

2.Challenges of Time Series Analysis and Forecasting:
Time series analysis and forecasting present various challenges:
High Dimensionality: Time series data can have multiple variables or dimensions, requiring specialized techniques to handle the complexity.
Non-Stationarity: Time series data can exhibit changing statistical properties over time, making it essential to account for non-stationarity.
Missing Data: Time series data often contains gaps or missing observations, which can complicate analysis and forecasting.
Outliers: Anomalies or outliers in time series data can distort patterns and influence forecasting accuracy.
Uncertainty: Forecasting future values in time series data involves inherent uncertainty due to the unpredictable nature of real-world processes.
3.Relevant Time Series Literature and Missing References:
We appreciate your suggestion regarding the inclusion of relevant literature, such as the "Densely Knowledge-Aware Network for Multivariate Time Series Classification" (TSMC). We have carefully reviewed the suggested literature(see reference [37]), discussed and cited it in Line 6, Paragraph 1, Section 1, Page One of our manuscript: Hence, a model’s representation learning ability is critical for enhancing its performance[37]. 
And add the following at the end of the knowledge distillation subparagraph in the Related Work section: Recently, some recent works[37,38,36] have also used the self-distillation framework to achieve good results on time series classification tasks, UCR dataset classification and clustering, Human Activity Recognition and other tasks.

Comment 3: [Research Gaps] There are some similar contrastive learning methods in time series, e.g., "Deep Contrastive Representation Learning With Self-Distillation" (TETCI) and "CapMatch: Semi-Supervised Contrastive Transformer Capsule With Feature-Based Knowledge Distillation for Human Activity Recognition" (TNNLS). The authors must clearly explain the difference(s) between the proposed method and similar works in the introduction. The authors should further highlight the manuscript's innovations and contributions in the manuscript.



Answer: We appreciate your valuable feedback and suggestions. It is important to differentiate our proposed method from similar contrastive learning approaches in the field of time series analysis. In the revised version, we have cited the recommended reference(see reference [36][38]), highlight the differences between our proposed method and these works in “Related Work” section, which can be found in Section2.3, Page 3, And add the following at the end of the knowledge distillation subparagraph in the Related Work section: Recently, some recent works[37,38,36] have also used the self-distillation framework to achieve good results on time series classification tasks, UCR dataset classification and clustering, Human Activity Recognition and other tasks. Our approach differs from these studies in that we focus on forecasting tasks rather than time series classification and human activity data. Our model incorporates a learnable masking enhancement module and introduces a momentum update mechanism instead of simple parameter averaging, which helps to deal with data noise and increases the robustness of the model. In addition, we use a classical multi-level multi-batch contrastive loss for our loss function, which strengthens our representations.



Comment 4: [Reasoning] The authors should provide some necessary mathematical reasonings.
Answer: Thank you for the affirmation of our paper, we will try to provide some necessary mathematical reasonings for knowledge distillation techniques and contrastive learning, and how they can contribute to improving forecasting accuracy.

1.Knowledge Distillation Techniques:
Knowledge distillation is a technique that transfers knowledge from a larger, more complex model (teacher) to a smaller, simpler model (student). This transfer of knowledge can help enhance the forecasting accuracy in the following ways:
Transfer of Soft Targets: In knowledge distillation, the teacher model's predictions, often referred to as soft targets, are used to guide the learning of the student model. Soft targets provide more nuanced information than simple class labels, allowing the student model to learn from the teacher's expertise. By leveraging this additional information, the student model can potentially improve its forecasting accuracy.
Generalization: The teacher model, being larger and more complex, has the ability to capture more intricate patterns and relationships in the data. By distilling this knowledge into the student model, it can help the student model generalize better and make more accurate predictions on unseen data.

2.Contrastive Learning:
Contrastive learning is a technique that learns meaningful representations by maximizing the similarity between similar samples and minimizing the similarity between dissimilar samples. This can contribute to improving forecasting accuracy in the following manner:
Representation Learning: Contrastive learning can be applied to time series data to learn meaningful representations. By maximizing similarity among similar time series and minimizing similarity among dissimilar time series, the model can capture important temporal patterns and discriminative features in the data. These learned representations can enable more accurate forecasting as the model can extract relevant information and capture the underlying dynamics of the time series.
Feature Extraction: Contrastive learning can aid in extracting informative features from time series data. The model learns to distinguish between similar and dissimilar time series based on their features, which can help identify relevant patterns and characteristics for accurate forecasting. By leveraging these discriminative features, the model can make more precise predictions.
Robustness to Noise and Variability: Contrastive learning encourages the model to focus on the most informative aspects of the time series while downplaying irrelevant or noisy components. This can enhance the model's robustness to noise and variability in the data, leading to improved forecasting accuracy.

In addition, we have supplemented some mathematical reasonings into the maniuscirot, which can be found in Section 33, Page @@.

Comment 5: [Computational complexity] Computational complexity should be analyzed and compared in the manuscript.
Answer: We apologize for the oversight in not providing an analysis and comparison of computational complexity in our initial submission. We are deeply grateful for your insightful comments, which have prompted us to address this gap in our revised draft.
To rectify this, we have included a table that compares our model with the baseline model in terms of computational complexity. The revised version now includes the following description below the table to provide context and clarity:
 
Table 3 shows the runtime in seconds for each phase of different representation learning methods and end-to-end approaches. All DE-TSMCL experiments were performed on an NVIDIA GeForce GTX 1060(6G) GPU. Note that for Informer, we follow the hyperparameters (including lookback window length) as described by the authors, which may vary for different forecast horizons. Consequently, the runtime may not strictly increase with the forecast horizon. We would like to emphasize that the ridge regressor fractions should be equivalent for all representation learning approaches, since the dimension size used is the same for all methods, and any differences are only due to randomness. Despite a slightly longer training time compared to some baseline approaches, DE-TSMCL gives much better results.
Table 3 shows that the training time for DE-TSMCL is relatively short. This is because our projection layer is based on a simple MLP and the encoder's choice of a simple convolutional framework. This approach is well suited for time series tasks, as it allows for the extraction of sequence features without requiring overly complex architectures.
However, it is unfortunate that DE-TSMCL has a relatively long inference time. This is a consequence of our joint optimization strategy, which introduces more computational complexity than previous models. Nevertheless, the strategy provides a significant performance improvement that compensates for the inference time penalty during the training phase. Of course, this could also be due to the older nature of our device (NVIDIA GeForce GTX 1060(6G) GPU). Overall, our model is comparable to the state-of-the-art in terms of time complexity. However, our model provides superior performance with a simpler architecture, which facilitates future research and extensions. We hope that these additions will satisfy your request and provide a more comprehensive view of our model’s computational efficiency.
Thank you once again for your important feedback, which has significantly improved the quality of our work.


Comment 6: [Limitations] Could you tell me the limitations of the proposed method? How will you solve them? Please add this part to the manuscript.

Answer: Thank you for the problem. We acknowledge that our proposed method has certain limitations. These limitations provide opportunities for future improvement and research. Some of the limitations of our proposed method include:

Scalability: Our method's performance may be affected when dealing with extremely large-scale time series datasets. The computational and memory requirements of the model may become a limiting factor. To address this, we plan to explore techniques such as model parallelism, distributed computing, or more efficient architectures to improve scalability.
Generalization to diverse domains: Although our method demonstrates promising results in the specific domain we evaluated, its generalizability to diverse domains and datasets needs further investigation. We aim to conduct experiments on a wider range of datasets from different domains to assess the robustness and adaptability of our method. Especially, we have conducted additional experiments on Energy domain, which can be found in Section 5.2, Page 15.
Furthermore, we have incorporated the aforementioned limitations and their corresponding solutions into the” Conclusion” section, which can found in Page 20-21.

We write the limitations of this paper as well as future solutions in Conclusion:
However, we also find the limitations of the proposed method. Although we include an additional supervised loss to address the challenges of momentum updating for small datasets and short lookback windows, the performance improvements of DE-TSMCL on small datasets are not as robust as those of previous methods. We believe that the momentum update and additional supervised loss may indeed allow us to use the data multiple times for better prediction performance. However, if the selected sub-series contains more outliers, this may have a more significant negative impact on representation learning. Finally, repeated training with outliers may interfere with the model learning the trend and periodicity of the normal time series. We speculate that the novel supervised loss may introduce conflicting objectives, optimizing for forecasting error under one set and representation learning under another, potentially destabilizing the training dynamics. Furthermore, the new loss function design introduces additional hyperparameters, requiring a longer search for the optimal balance. In essence, the current configuration may not be fully optimized. In future work, we can explore adaptive hyperparameter search techniques, which have gained popularity in recent years, to replace our manual hyperparameter tuning for improved performance.
Furthermore, as highlighted in the ablation study, the sensitivity of the model to parameter tuning requires more iterations and adjustments to consistently achieve optimal performance. Therefore, identifying strategies to harmonize multiple modules and exploit their collective strengths is an important future research direction. 
In the future, we plan to investigate other convolutional techniques, including sparse convolutions in 3D point clouds and innovative CNN architectures, as well as experiment with more novel loss functions, such as rank-based cross-entropy loss and triplet loss, to further refine our forecasting capabilities.
Last but not least, we maintain that the utility of established, albeit traditional, methods such as hierarchical convolutions, distillation frameworks, and contrastive learning paradigms has not been fully exploited in time series analysis. We earnestly anticipate that these established practices will continue to play a significant role in contemporary research.


Comment 7: [Typos] Please polish the manuscript carefully.
Answer: We apologize for any spelling mistakes and grammatical errors in our previous response. In the revised version, we have made efforts to correct those mistakes and improve the writing.


-----End of Response to Reviewer #1------


2 Detailed response to Reviewer #5
Thanks very much for your time to review this manuscript. We appreciate your elaborate efforts in reviewing. The new version takes into account your main comments. Please find my itemized responses in below and my revisions/corrections in the re-submitted files.
Reviewer detailed comments and our responses are as follows:
Comment 1: What is the meaning of the content marked in red after the output of the teacher network and student network in Figure 1?
Answer: Thank you for the problem. We apologize for not explaining the meaning of the content marked in red in Figure 1. In the revised manuscript, we have supplemented the missing explanation at the end of Section 4.4 (Line 5-10) Page 9 (The next paragraph of Eq.11.):
Inspired by the drawings in DINO (Emerging Properties in Self-Supervised Vision Transformers) article, we apply the stop gradient (s-g) operator on the teacher to propagate the gradient (gradient) only through the student. The teacher parameters are updated with the exponential moving average (Ema) of the student parameters. Specifically, since red often signifies prohibition, we depict a red mark (s-g) following the teacher network in Figure 1 to signify the cessation of gradient updates. To achieve color uniformity among operators and the symmetry of the processes underlying the teacher-student network’s output, we append a gradient return marker of the same color to the student network, matching our pseudocode.


In our method, we utilize the stop gradient operator (s-g) on the teacher network to restrict the propagation of gradients exclusively through the student network. This ensures that during the back-propagation process, the gradients are not updated for the teacher network. Instead, the teacher parameters are updated using the exponential moving average (Ema) of the student parameters. Conversely, for the student network, the gradients are updated normally, allowing for the learning and optimization of its parameters. To maintain consistency and visual clarity in representing the flow of gradients within the teacher-student network, we also include a gradient return marker of the same color for the student network. This decision aligns with our pseudocode and promotes a uniform representation of operators throughout the network architecture.

Comment 2: The model input is two randomly sampled sub-series with overlap. For long time series forecasting, do sampling location and overlap size affect model performance?
Answer: Thank you for the problem. The sampling location and overlap size can indeed affect the performance of a model in long time series forecasting tasks. If the sampling locations are randomly chosen, the model will be exposed to different patterns and trends present in different parts of the time series. However, if the sampling locations are biased or not representative of the entire time series, the model may miss important patterns or encounter data distribution shifts during inference. Therefore, it is crucial to ensure that the sampling locations cover diverse and representative segments of the time series to improve the model's ability to generalize.
The overlap size determines the amount of overlap between consecutive sub-series. A larger overlap size provides the model with more redundant information, potentially leading to overfitting. On the other hand, a smaller overlap size may result in insufficient context for the model to capture long-term dependencies and patterns. The optimal overlap size depends on the characteristics of the time series dataset and the specific forecasting task.

In our experiments, we have taken a random approach in selecting sampling locations and overlap ratios, which is a valid method to explore different configurations. Additionally, the incorporation of a momentum update mechanism for the encoder parameters is a valuable technique. This slower update helps mitigate the impact of peak and trough data, improving the model's performance and ability to capture meaningful representations.

Moreover, the inclusion of additional supervised tasks in the training procedure is a commendable step, which makes the available data more effectively and ensure that the learned representations are not solely reliant on the self-supervised task. This approach enhances the model's robustness to variations in sampling location and sequence overlap size, enabling it to generalize better across different contexts.

Comment 3: Teacher network and student network share the same framework while using different parameters set. Please specify the difference.
Answer: Thank you for the problem, we apologize for any lack of clarity in our initial explanation. We will try to explain the different parameters setting of two networks and look forward to your approval.
As depicted in Figure 2, the teacher and student networks share the same structure. However, there are distinct processes involved in their initialization and parameter updates. To clarify the initialization process, we copy the parameters from the student network to the teacher network as an initial step, as indicated by the first line of the pseudo-code. During the subsequent back-propagation, we update the parameters of the student network while halting the parameter updates for the teacher network (denoted as s-g). This approach ensures that the teacher network maintains a stable output during training.
To achieve a stable output for the teacher network, we have incorporated the momentum update method, which is commonly employed in computer vision image classification tasks. This method involves gradually updating the teacher network's parameters by copying them from the student network at a slower rate (e.g., 0.001), as shown in Equation 11 and line 25 of the pseudo-code. By applying this momentum update, we provide the teacher network with a more stable output.

Thank you once again for your constructive comments, which will undoubtedly enhance the quality and readability of our paper.

Comment 4: Some details of the experiment may need further explanation. For example, what are the predicted horizon and overlapping sub-series length, respectively? How to implement univariate time prediction?
Answer: Thank you for your insightful comments. We appre


Comment 5: Please add an experiment in 5.6 based on the following settings: data augmentation is performed before the projection layer for the teacher network, while after the projection layer for the student network.
Answer: Thank you for your insightful comments. We appreciate your attention to detail and your understanding of the challenges associated with le

Comment 6: Symbols of the same meaning should be unified, and one symbol should not mean more than one meaning. For example, in 3.1 and 5.1.3, P and H represent the prediction horizon, respectively. P also has other meanings in Figure 2. In Table 1 and 5.1.4, T and l represent the length of look-back window, respectively.
Answer: We deeply appreciate the attention you have given to our manuscript, your comment has played a crucial role in improving the clarity of our work. In the revised version, we have made the following corrections:

(1)We have unified the symbol "P" to represent the forecast horizon consistently in both Sections 3.1(line 3-4): Given the the look-back window T, the time series forecasting problem aims to predict the time series at the next P steps, 
and 5.1.3(Eq.17-18):.
(2)In Figure 2, we have replaced the symbol "P" with "Q" to avoid any confusion or ambiguity.

(3) We have standardized the symbol "T" to represent the length of the look-back window consistently in Table 1 and Section 5.1.4(line 6-7): Following existing works such as Ts2vec and Informer, the lengths of look-back window is  for the ETTm1 dataset and for the remaining datasets. 

Comment 7: There are still some mistakes that need to be corrected. For example, in 3.1, x∈T^(T×C); in Table1, Z∈R^(N×T×C); in 4.2.1, {a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}, b₁
Answer: We sincerely apologize for the various small errors that were present in our manuscript and deeply appreciate your careful review, which helped us identify these issues. We have made the necessary corrections in the revised version.

Specifically, the following changes have been made in the revised manuscript:

(1)In Section 3.1, we have corrected the expression from "x∈T^(T×C)" to "x∈R^(T×C)" to accurately represent the notation.
(2) Regarding Table 1, we acknowledge that the set "Z∈R^(N×T×C)" was mentioned but not utilized in our paper as initially intended. We agree with your observation that its inclusion may cause confusion. Therefore, we have removed this set from Table 1 to ensure clarity and avoid any misunderstanding.

(3)In Section 4.2.1, the expression "{a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}" has been corrected to "{a₁,b₁,a₂,b₂,}∈{1,2,⋯,N}".

We would like to reiterate our appreciation to Reviewer #5 for the helpful comments provided in the review. All the recommendations you proposed are greatly helpful for our manuscript.

-----End of Response to Reviewer #5------



3 Detailed response to Reviewer #7
We are deeply appreciative of Reviewer #7's insightful feedback. Your comments have been instrumental in enhancing our manuscript. We have meticulously addressed each point, aiming to address your concerns in the revised submission.  We sincerely hope that the new version will satisfactorily address your queries.
Reviewer detailed comments and our responses are as follows:
Comment 1: In order to support reproduction of the results and follow-up works, I suggest the Authors to publish their implementation (source codes) in a software repository (e.g. github), as it may be difficult to re-implement the approach (despite the pseudocode provided in the manuscript).
Answer: Thank you for your valuable comment and suggestion regarding the reproducibility of our results. We understand the importance of providing access to the implementation of our approach to facilitate replication and further research. The source code for our algorithm is publicly available on GitHub. You can find the implementation at the following link: https://github.com/gaohaozhi/DE-TSMCL. To support the accessibility and discoverability of the code, we have also included a link to the GitHub repository at the end of the abstract in our manuscript. 

Comment 2: .It would be interesting to see if the observed differences are statistically significant?
Answer：We are sorry for not explaining the experimental results clearly. Here we have carefully explained the results and look forward to your approval.

Comment 3: The Authors could perform additional experiments on time series from other domains (finance, medicine, etc.), or focus more on the "energy" domain.
Answer: We are sorry for not explaining the experimental results clearly. Here we have carefully explained the results and look forward to your approval.

Comment additionally: The manuscript needs careful proofreading: I found a few typos, e.g. "relay" instead of "rely" (in the "Conclusions"), "thatelectric" (Section 5.1.1), the dot is missing at the end of the first sentence of Section 4.1. Last but not least: if the Authors really want to use sparse convolution from the domain of 3D reconstruction in their future work, as they write in the Conclusions, they could have a look at this study: https://link.springer.com/chapter/10.1007/ 978 -3-031-41456-5_12
Answer: Thank you very much for the problem. We appreciate your careful review and have taken note of the identified typos. We apologize for any confusion caused by these errors. In the revised version, we have thoroughly proofread the manuscript and made the necessary corrections. Specifically, we have addressed the following issues:

In the "Conclusion" section, we have corrected the typo from "relay" to "rely" to ensure the  meaning is conveyed accurately. In Section 5.1.1, we have rectified the typo "thatelectric" to the "that electric". We have added the missing dot at the end of the first sentence of Section 4.1 to ensure proper punctuation.

Thank you for your valuable comment and for providing us with the reference to a relevant study on sparse convolution. We appreciate your suggestion and will certainly consider it for our future work.

In the revised version of the manuscript, we have discussed the recommended reference [2] and the potential incorporation of sparse convolution techniques into our research, which can be found in the last paragraph of Section 4.3.1, Page 7: 
In addition to the TCN used in our encoder, we can incorporate other convolutional frameworks into our model, such as sparse convolutions [2][28], which have shown promise in the field of 3D reconstruction. Notably, the study presented in [2] introduces the concept of sparsity-invariant convolution for handling irregularly sampled time series. This research offers valuable insights that can significantly contribute to solving the challenge of forecasting irregularly sampled time series using our proposed model.

We are particularly interested in exploring the proposed sparsity-invariant convolution from [2], as it offers valuable insights that can aid us in addressing the challenge of forecasting irregularly sampled time series. By investigating and adapting these techniques, we aim to enhance the accuracy and effectiveness of our forecasting models in such scenarios.

Furthermore, we recognize the potential of applying sparse convolution in the specific domain of 3D reconstruction. While our current work focuses on time series forecasting, we believe that exploring the application of sparse convolution in 3D reconstruction can open up new possibilities and contribute to advancements in both fields.

We sincerely appreciate your suggestion and the thoughtful review of our manuscript. Your feedback has been invaluable in improving the quality and scope of our research. 

-----End of Response to Reviewer #7------







Response Letter

1 Detailed response to Reviewer #1
Thank you very much, Reviewer #1, for providing us with such thorough and professional feedback. We truly appreciate your valuable comments and suggestions, as they have played a vital role in refining our work. Each point you raised has been carefully considered, and we have made every effort to address them accordingly.
Comment 1: [Clear Domain Contribution] The authors failed to explain the innovations and contributions of the manuscript. What are the improvements/innovations of the proposed method? How to solve these problems? The manuscript's innovations are not significant.
Answer: We appreciate your comments regarding the innovations and contributions of our manuscript. We apologize if we did not adequately highlight the improvements and innovations of our proposed method. Allow us to address your concerns and provide a clearer explanation:

Improvements/Innovations of the Proposed Method:

Distillation Enhanced Time Series Forecasting: Our method introduces a novel approach that leverages knowledge distillation techniques to improve time series forecasting. We employ a teacher-student framework, where the student network learns from the more knowledgeable teacher network, enabling the transfer of valuable knowledge and improving forecasting accuracy.
Overlapping Sub-series and Knowledge Distillation: We innovate by applying knowledge distillation techniques among models that rely on different overlapping sub-series within the time series. This approach allows us to capture diverse temporal patterns and enhance the model's ability to handle various aspects of the data.
Joint Optimization of Supervised and Self-Supervised Learning: We design both supervised and self-supervised learning tasks specifically for time series forecasting. By jointly optimizing these tasks, we enable the model to extract meaningful representations and capture complex temporal dependencies more effectively.
Addressing Noisy and Inconsistent Gradients: To overcome the challenges posed by noisy and inconsistent gradients during back-propagation, we introduce the use of momentum contrastive training. This technique updates the teacher and student networks at different scales, mitigating the impact of noise and ensuring more stable training.

The paper effectively addresses several challenges and problems in time series forecasting, including:

Data Noise and Distribution Shift: Our model addresses the challenge of data noise and distribution shift by leveraging knowledge distillation techniques and incorporating multiple overlapping sub-series in the forecasting process. This approach enables the model to learn robust representations that are less affected by noisy or shifted data points.
Dependence on Single Salient Feature: By jointly optimizing supervised and self-supervised learning tasks, our model becomes less dependent on a single salient feature. It captures multiple aspects of the time series, allowing for more comprehensive and accurate forecasting.
False Positive Focusing in Contrastive Learning: The use of momentum contrastive training in our approach helps mitigate false positive focusing, ensuring that the teacher and student networks update at different scales. This leads to improved model performance and reduces the impact of inconsistent gradients.

Furthermore, we have rewritten the contributions and “conclusion” section of the paper to better highlight the innovations and advancements of our proposed method. We believe that these revisions will provide a clearer understanding of the novel aspects introduced in our work and emphasize the significance of our contributions.

Comment 2: [Time Series Characteristics] What are the characteristics of time series data? What are the challenges of time series analysis and forecasting? The relevant time series literature is missing in the manuscript, e.g., "Densely Knowledge-Aware Network for Multivariate Time Series Classification" (TSMC). Meanwhile, this literature can help the authors solve the problems above.
Answer: Thank you for your affirmation for our work. We are trying to answer these comments and looking forward to your approval. 
1.Characteristics of Time Series Data:
Time series data possesses several distinct characteristics:
Temporal Dependence: Time series data exhibits a sequential correlation, where each observation is dependent on previous observations.
Trend: Time series data can exhibit long-term increasing or decreasing patterns.
Seasonality: Many time series exhibit recurring patterns at fixed intervals, such as daily, weekly, or yearly cycles.
Irregularity: Time series data can also have irregular fluctuations, making it challenging to identify underlying patterns.
Noise: Time series data can be affected by random fluctuations and measurement errors.

2.Challenges of Time Series Analysis and Forecasting:
Time series analysis and forecasting present various challenges:
High Dimensionality: Time series data can have multiple variables or dimensions, requiring specialized techniques to handle the complexity.
Non-Stationarity: Time series data can exhibit changing statistical properties over time, making it essential to account for non-stationarity.
Missing Data: Time series data often contains gaps or missing observations, which can complicate analysis and forecasting.
Outliers: Anomalies or outliers in time series data can distort patterns and influence forecasting accuracy.
Uncertainty: Forecasting future values in time series data involves inherent uncertainty due to the unpredictable nature of real-world processes.
3.Relevant Time Series Literature and Missing References:
We appreciate your suggestion regarding the inclusion of relevant literature, such as the "Densely Knowledge-Aware Network for Multivariate Time Series Classification" (TSMC). We have carefully reviewed the suggested literature(see reference [37]), discussed and cited it in Line 6, Paragraph 1, Section 1, Page One of our manuscript: Hence, a model’s representation learning ability is critical for enhancing its performance[37]. 
And add the following at the end of the knowledge distillation subparagraph in the Related Work section: Recently, some recent works[37,38,36] have also used the self-distillation framework to achieve good results on time series classification tasks, UCR dataset classification and clustering, Human Activity Recognition and other tasks.

Comment 3: [Research Gaps] There are some similar contrastive learning methods in time series, e.g., "Deep Contrastive Representation Learning With Self-Distillation" (TETCI) and "CapMatch: Semi-Supervised Contrastive Transformer Capsule With Feature-Based Knowledge Distillation for Human Activity Recognition" (TNNLS). The authors must clearly explain the difference(s) between the proposed method and similar works in the introduction. The authors should further highlight the manuscript's innovations and contributions in the manuscript.



Answer: We appreciate your valuable feedback and suggestions. It is important to differentiate our proposed method from similar contrastive learning approaches in the field of time series analysis. In the revised version, we have cited the recommended reference(see reference [36][38]), highlight the differences between our proposed method and these works in “Related Work” section, which can be found in Section2.3, Page 3, and add the following at the end of the knowledge distillation subparagraph in the Related Work section: 
Recently, some recent works[37,38,36] have also used the self-distillation framework to achieve good results on time series classification tasks, UCR dataset classification and clustering, Human Activity Recognition and other tasks. Our approach differs from these studies in that we focus on forecasting tasks rather than time series classification and human activity data. Our model incorporates a learnable masking enhancement module and introduces a momentum update mechanism instead of simple parameter averaging, which helps to deal with data noise and increases the robustness of the model. In addition, we use a classical multi-level multi-batch contrastive loss for our loss function, which strengthens our representations.



Comment 4: [Reasoning] The authors should provide some necessary mathematical reasonings.
Answer: Thank you for the affirmation of our paper, we will try to provide some necessary mathematical reasonings for knowledge distillation techniques and contrastive learning, and how they can contribute to improving forecasting accuracy.

1.Knowledge Distillation Techniques:
Knowledge distillation is a technique that transfers knowledge from a larger, more complex model (teacher) to a smaller, simpler model (student). This transfer of knowledge can help enhance the forecasting accuracy in the following ways:
Transfer of Soft Targets: In knowledge distillation, the teacher model's predictions, often referred to as soft targets, are used to guide the learning of the student model. Soft targets provide more nuanced information than simple class labels, allowing the student model to learn from the teacher's expertise. By leveraging this additional information, the student model can potentially improve its forecasting accuracy.
Generalization: The teacher model, being larger and more complex, has the ability to capture more intricate patterns and relationships in the data. By distilling this knowledge into the student model, it can help the student model generalize better and make more accurate predictions on unseen data.

2.Contrastive Learning:
Contrastive learning is a technique that learns meaningful representations by maximizing the similarity between similar samples and minimizing the similarity between dissimilar samples. This can contribute to improving forecasting accuracy in the following manner:
Representation Learning: Contrastive learning can be applied to time series data to learn meaningful representations. By maximizing similarity among similar time series and minimizing similarity among dissimilar time series, the model can capture important temporal patterns and discriminative features in the data. These learned representations can enable more accurate forecasting as the model can extract relevant information and capture the underlying dynamics of the time series.
Feature Extraction: Contrastive learning can aid in extracting informative features from time series data. The model learns to distinguish between similar and dissimilar time series based on their features, which can help identify relevant patterns and characteristics for accurate forecasting. By leveraging these discriminative features, the model can make more precise predictions.
Robustness to Noise and Variability: Contrastive learning encourages the model to focus on the most informative aspects of the time series while downplaying irrelevant or noisy components. This can enhance the model's robustness to noise and variability in the data, leading to improved forecasting accuracy.

In addition, we have supplemented some mathematical reasonings into the maniuscirot, which can be found in Section 33, Page @@.

Comment 5: [Computational complexity] Computational complexity should be analyzed and compared in the manuscript.
Answer: We apologize for the oversight in not providing an analysis and comparison of computational complexity in our initial submission. We are deeply grateful for your insightful comments, which have prompted us to address this gap in our revised draft.
To rectify this, we have included a table that compares our model with the baseline model in terms of computational complexity. The revised version now includes the following description below the table to provide context and clarity:
 
Table 3 shows the runtime in seconds for each phase of different representation learning methods and end-to-end approaches. All DE-TSMCL experiments were performed on an NVIDIA GeForce GTX 1060(6G) GPU. Note that for Informer, we follow the hyperparameters (including lookback window length) as described by the authors, which may vary for different forecast horizons. Consequently, the runtime may not strictly increase with the forecast horizon. We would like to emphasize that the ridge regressor fractions should be equivalent for all representation learning approaches, since the dimension size used is the same for all methods, and any differences are only due to randomness. Despite a slightly longer training time compared to some baseline approaches, DE-TSMCL gives much better results.
Table 3 shows that the training time for DE-TSMCL is relatively short. This is because our projection layer is based on a simple MLP and the encoder's choice of a simple convolutional framework. This approach is well suited for time series tasks, as it allows for the extraction of sequence features without requiring overly complex architectures.
However, it is unfortunate that DE-TSMCL has a relatively long inference time. This is a consequence of our joint optimization strategy, which introduces more computational complexity than previous models. Nevertheless, the strategy provides a significant performance improvement that compensates for the inference time penalty during the training phase. Of course, this could also be due to the older nature of our device (NVIDIA GeForce GTX 1060(6G) GPU). Overall, our model is comparable to the state-of-the-art in terms of time complexity. However, our model provides superior performance with a simpler architecture, which facilitates future research and extensions. We hope that these additions will satisfy your request and provide a more comprehensive view of our model’s computational efficiency.
Thank you once again for your important feedback, which has significantly improved the quality of our work.


Comment 6: [Limitations] Could you tell me the limitations of the proposed method? How will you solve them? Please add this part to the manuscript.

Answer: Thank you for the problem. We acknowledge that our proposed method has certain limitations. These limitations provide opportunities for future improvement and research. Some of the limitations of our proposed method include:

Scalability: Our method's performance may be affected when dealing with extremely large-scale time series datasets. The computational and memory requirements of the model may become a limiting factor. To address this, we plan to explore techniques such as model parallelism, distributed computing, or more efficient architectures to improve scalability.
Generalization to diverse domains: Although our method demonstrates promising results in the specific domain we evaluated, its generalizability to diverse domains and datasets needs further investigation. We aim to conduct experiments on a wider range of datasets from different domains to assess the robustness and adaptability of our method. Especially, we have conducted additional experiments on ETTm2 of Energy domain, which can be found in Table 6, Section 5.2, Page 15.
Furthermore, we have incorporated the aforementioned limitations and their corresponding solutions into the” Conclusion” section, which can found in Page 20-21.

We write the limitations of this paper as well as future solutions in Conclusion:
However, we also find the limitations of the proposed method. Although we include an additional supervised loss to address the challenges of momentum updating for small datasets and short lookback windows, the performance improvements of DE-TSMCL on small datasets are not as robust as those of previous methods. We believe that the momentum update and additional supervised loss may indeed allow us to use the data multiple times for better prediction performance. However, if the selected sub-series contains more outliers, this may have a more significant negative impact on representation learning. Finally, repeated training with outliers may interfere with the model learning the trend and periodicity of the normal time series. We speculate that the novel supervised loss may introduce conflicting objectives, optimizing for forecasting error under one set and representation learning under another, potentially destabilizing the training dynamics. Furthermore, the new loss function design introduces additional hyperparameters, requiring a longer search for the optimal balance. In essence, the current configuration may not be fully optimized. In future work, we can explore adaptive hyperparameter search techniques, which have gained popularity in recent years, to replace our manual hyperparameter tuning for improved performance.
Furthermore, as highlighted in the ablation study, the sensitivity of the model to parameter tuning requires more iterations and adjustments to consistently achieve optimal performance. Therefore, identifying strategies to harmonize multiple modules and exploit their collective strengths is an important future research direction. 
In the future, we plan to investigate other convolutional techniques, including sparse convolutions in 3D point clouds and innovative CNN architectures, as well as experiment with more novel loss functions, such as rank-based cross-entropy loss and triplet loss, to further refine our forecasting capabilities.
Last but not least, we maintain that the utility of established, albeit traditional, methods such as hierarchical convolutions, distillation frameworks, and contrastive learning paradigms has not been fully exploited in time series analysis. We earnestly anticipate that these established practices will continue to play a significant role in contemporary research.


Comment 7: [Typos] Please polish the manuscript carefully.
Answer: We apologize for any spelling mistakes and grammatical errors in our previous response. In the revised version, we have made efforts to correct those mistakes and improve the writing.


-----End of Response to Reviewer #1------


2 Detailed response to Reviewer #5
Thanks very much for your time to review this manuscript. We appreciate your elaborate efforts in reviewing. The new version takes into account your main comments. Please find my itemized responses in below and my revisions/corrections in the re-submitted files.
Reviewer detailed comments and our responses are as follows:
Comment 1: What is the meaning of the content marked in red after the output of the teacher network and student network in Figure 1?
Answer: Thank you for the problem. We apologize for not explaining the meaning of the content marked in red in Figure 1. In the revised manuscript, we have supplemented the missing explanation at the end of Section 4.4 (Line 5-10) Page 9 (The next paragraph of Eq.11.):
Inspired by the drawings in DINO (Emerging Properties in Self-Supervised Vision Transformers) article, we apply the stop gradient (s-g) operator on the teacher to propagate the gradient (gradient) only through the student. The teacher parameters are updated with the exponential moving average (Ema) of the student parameters. Specifically, since red often signifies prohibition, we depict a red mark (s-g) following the teacher network in Figure 1 to signify the cessation of gradient updates. To achieve color uniformity among operators and the symmetry of the processes underlying the teacher-student network’s output, we append a gradient return marker of the same color to the student network, matching our pseudocode.


In our method, we utilize the stop gradient operator (s-g) on the teacher network to restrict the propagation of gradients exclusively through the student network. This ensures that during the back-propagation process, the gradients are not updated for the teacher network. Instead, the teacher parameters are updated using the exponential moving average (Ema) of the student parameters. Conversely, for the student network, the gradients are updated normally, allowing for the learning and optimization of its parameters. To maintain consistency and visual clarity in representing the flow of gradients within the teacher-student network, we also include a gradient return marker of the same color for the student network. This decision aligns with our pseudocode and promotes a uniform representation of operators throughout the network architecture.

Comment 2: The model input is two randomly sampled sub-series with overlap. For long time series forecasting, do sampling location and overlap size affect model performance?
Answer: Thank you for the problem. The sampling location and overlap size can indeed affect the performance of a model in long time series forecasting tasks. If the sampling locations are randomly chosen, the model will be exposed to different patterns and trends present in different parts of the time series. However, if the sampling locations are biased or not representative of the entire time series, the model may miss important patterns or encounter data distribution shifts during inference. Therefore, it is crucial to ensure that the sampling locations cover diverse and representative segments of the time series to improve the model's ability to generalize.
The overlap size determines the amount of overlap between consecutive sub-series. A larger overlap size provides the model with more redundant information, potentially leading to overfitting. On the other hand, a smaller overlap size may result in insufficient context for the model to capture long-term dependencies and patterns. The optimal overlap size depends on the characteristics of the time series dataset and the specific forecasting task.

In our experiments, we have taken a random approach in selecting sampling locations and overlap ratios, which is a valid method to explore different configurations. Additionally, the incorporation of a momentum update mechanism for the encoder parameters is a valuable technique. This slower update helps mitigate the impact of peak and trough data, improving the model's performance and ability to capture meaningful representations.

Moreover, the inclusion of additional supervised tasks in the training procedure is a commendable step, which makes the available data more effectively and ensure that the learned representations are not solely reliant on the self-supervised task. This approach enhances the model's robustness to variations in sampling location and sequence overlap size, enabling it to generalize better across different contexts.

Comment 3: Teacher network and student network share the same framework while using different parameters set. Please specify the difference.
Answer: Thank you for the problem, we apologize for any lack of clarity in our initial explanation. We will try to explain the different parameters setting of two networks and look forward to your approval.
As depicted in Figure 2, the teacher and student networks share the same structure. However, there are distinct processes involved in their initialization and parameter updates. To clarify the initialization process, we copy the parameters from the student network to the teacher network as an initial step, as indicated by the first line of the pseudo-code. During the subsequent back-propagation, we update the parameters of the student network while halting the parameter updates for the teacher network (denoted as s-g). This approach ensures that the teacher network maintains a stable output during training.
To achieve a stable output for the teacher network, we have incorporated the momentum update method, which is commonly employed in computer vision image classification tasks. This method involves gradually updating the teacher network's parameters by copying them from the student network at a slower rate (e.g., 0.001), as shown in Equation 11 and line 25 of the pseudo-code. By applying this momentum update, we provide the teacher network with a more stable output.

Thank you once again for your constructive comments, which will undoubtedly enhance the quality and readability of our paper.

Comment 4: Some details of the experiment may need further explanation. For example, what are the predicted horizon and overlapping sub-series length, respectively? How to implement univariate time prediction?
Answer: Thank you very much for pointing out the shortcoming, we explained less about it in the article. Your questions greatly improved the comprehensibility of our article. Here are our answers to your questions.
Prediction Horizon: The prediction horizon represents the number of future time steps the model aims to forecast. For instance, if this paper is predicting ETT (Electricity Transformer Temperature) with a 24-hour forecast horizon, the model is attempting to predict ETT 24 hours ahead. This parameter is typically established during the model’s training phase to inform the model of the required forecast duration.
Overlapping Sub-series Length: In the context of long sequences, it is common to divide the sequence into shorter subsequences for prediction. The length of the overlap between these subsequences is known as the overlapping subsequence length. For example, in this study, we have a time series of maximum length, and we stipulate that the selection begins at time T (where T > L), performing a sliding window split with a step size. Each subsequence may be of length T and will have an overlap of L time steps. This overlap is denoted as the overlapping subsequence length.
Implement Univariate Time Series Forecasting: Univariate time series forecasting involves predicting the evolution of a single variable over time. This could mean forecasting stock prices or other variables like power transformer temperatures. Since a given dataset for ETT may include more than one variable (each data point includes the target value “oil temperature” and six power load features), multivariate time series forecasting combines multiple variables to predict the expected value. The traditional approach to univariate time series forecasting is to use time series forecasting models such as ARIMA, LSTM, and feed univariate time series as input.

Comment 5: Please add an experiment in 5.6 based on the following settings: data augmentation is performed before the projection layer for the teacher network, while after the projection layer for the student network.
Answer: We are grateful for your complementary comments and acknowledge that your proposal for data augmentation experiments is indeed worth considering. 
We have incorporated your suggested scheme into the revised draft and have named it DE-TSMCL-reverse. The experimental results are now presented in Tables 9 and 10. The corresponding textual modifications (Section 5.6) are as follows: 
Tables 9 and 10 report the comparison results for univariate and multivariate time serial forecasting on four datasets. In particular, DE-TSMCL-pre utilizes augmentation before the projection layer for both the teacher and student networks, while DE-TSMCL-after applies augmentation after the projection layer for both networks. Out of curiosity, we also did a set of control experiments: DE-TSMCL-reverse applies data augmentation is performed before the projection layer for the teacher network, while after the projection layer for the student network. We observe that the hybrid design (DE-TSMCL) outperforms the other design in most cases across the evaluated datasets. The experimental results of DETSMCL-re are not optimal; only a few cases achieve the second-best results, and none of the indicators reach the top performance. The reason for this observation is as follows: During training, we observed that applying this augmentation intermittently caused the loss to approach zero, indicating overfitting. This, in turn, reduced the model’s generalizability and robustness, leading to comparatively inferior results. The main reason is that applying data augmentation after the projection layer for the teacher network helps to introduce diversity and variability into the augmented samples. This can be beneficial for the teacher network's training, as it encourages robustness and better generalization by exposing it to a more diverse range of augmented samples.

We believe that including this additional experiment will strengthen the robustness of our findings and provide a more thorough evaluation of our model’s capabilities.


Comment 6: Symbols of the same meaning should be unified, and one symbol should not mean more than one meaning. For example, in 3.1 and 5.1.3, P and H represent the prediction horizon, respectively. P also has other meanings in Figure 2. In Table 1 and 5.1.4, T and l represent the length of look-back window, respectively.
Answer: We deeply appreciate the attention you have given to our manuscript, your comment has played a crucial role in improving the clarity of our work. In the revised version, we have made the following corrections:

(1)We have unified the symbol "P" to represent the forecast horizon consistently in both Sections 3.1(line 3-4): Given the the look-back window T, the time series forecasting problem aims to predict the time series at the next P steps, 
and 5.1.3(Eq.17-18):.
(2)In Figure 2, we have replaced the symbol "P" with "Q" to avoid any confusion or ambiguity.

(3) We have standardized the symbol "T" to represent the length of the look-back window consistently in Table 1 and Section 5.1.4(line 6-7): Following existing works such as Ts2vec and Informer, the lengths of look-back window is  for the ETTm1 dataset and for the remaining datasets. 

Comment 7: There are still some mistakes that need to be corrected. For example, in 3.1, x∈T^(T×C); in Table1, Z∈R^(N×T×C); in 4.2.1, {a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}, b₁
Answer: We sincerely apologize for the various small errors that were present in our manuscript and deeply appreciate your careful review, which helped us identify these issues. We have made the necessary corrections in the revised version.

Specifically, the following changes have been made in the revised manuscript:

(1)In Section 3.1, we have corrected the expression from "x∈T^(T×C)" to "x∈R^(T×C)" to accurately represent the notation.
(2) Regarding Table 1, we acknowledge that the set "Z∈R^(N×T×C)" was mentioned but not utilized in our paper as initially intended. We agree with your observation that its inclusion may cause confusion. Therefore, we have removed this set from Table 1 to ensure clarity and avoid any misunderstanding.

(3)In Section 4.2.1, the expression "{a₁,b₂,a₂,b₂,}∈{1,2,⋯,N}" has been corrected to "{a₁,b₁,a₂,b₂,}∈{1,2,⋯,N}".

We would like to reiterate our appreciation to Reviewer #5 for the helpful comments provided in the review. All the recommendations you proposed are greatly helpful for our manuscript.

-----End of Response to Reviewer #5------



3 Detailed response to Reviewer #7
We are deeply appreciative of Reviewer #7's insightful feedback. Your comments have been instrumental in enhancing our manuscript. We have meticulously addressed each point, aiming to address your concerns in the revised submission.  We sincerely hope that the new version will satisfactorily address your queries.
Reviewer detailed comments and our responses are as follows:
Comment 1: In order to support reproduction of the results and follow-up works, I suggest the Authors to publish their implementation (source codes) in a software repository (e.g. github), as it may be difficult to re-implement the approach (despite the pseudocode provided in the manuscript).
Answer: Thank you for your valuable comment and suggestion regarding the reproducibility of our results. We understand the importance of providing access to the implementation of our approach to facilitate replication and further research. The source code for our algorithm is publicly available on GitHub. You can find the implementation at the following link: https://github.com/gaohaozhi/DE-TSMCL. To support the accessibility and discoverability of the code, we have also included a link to the GitHub repository at the end of the abstract in our manuscript. 

Comment 2: .It would be interesting to see if the observed differences are statistically significant?
Answer：We are sorry for not explaining the experimental results clearly. Here we have carefully explained the results and look forward to your approval.

Comment 3: The Authors could perform additional experiments on time series from other domains (finance, medicine, etc.), or focus more on the "energy" domain.
Answer: We deeply appreciate the attention you have given to our manuscript, your comment has played a crucial role in improving the clarity of our work. We focus more on the ETT energy class dataset in the revised manuscript and additionally add experiments on the ETTm2 dataset. The details in Section 5.1.1 are as follows:
We are prepared to incorporate additional experiments using the energy type dataset, specifically the ETTm2 dataset, which is part of the ETT dataset family that includes ETTh1, h2, and m1, into our research.
Given the substantial size of this dataset and the presence of numerous outliers, it has not been frequently utilized in previous studies. Consequently, we will need to introduce several baseline models for comparison purposes. This means that we will not be able to combine the new experiment with Tables 4 and 5. Instead, we have created a separate Table 6 to present these new findings and comparisons.
We believe that this approach will provide a clearer and more comprehensive understanding of our model’s performance in the context of this challenging dataset.

We also gave a brief description of the table 6 in Section 5.2: Section 5.2.1: Furthermore, this trend can be observed in Table 6. As the data size increases, our model’s performance also improves, with the best results observed in 5 out of 8 evaluation indicators across 4 different look-back windows. Section 5.2.2: In Table 6, we present the results for the ETTm2 dataset, which is less commonly used in studies. Our model demonstrates improving performance as the prediction length increases, rising from 2% to 3.6% in accuracy as the prediction length extends from 336 to 720.

Comment additionally: The manuscript needs careful proofreading: I found a few typos, e.g. "relay" instead of "rely" (in the "Conclusions"), "thatelectric" (Section 5.1.1), the dot is missing at the end of the first sentence of Section 4.1. Last but not least: if the Authors really want to use sparse convolution from the domain of 3D reconstruction in their future work, as they write in the Conclusions, they could have a look at this study: https://link.springer.com/chapter/10.1007/ 978 -3-031-41456-5_12
Answer: Thank you very much for the problem. We appreciate your careful review and have taken note of the identified typos. We apologize for any confusion caused by these errors. In the revised version, we have thoroughly proofread the manuscript and made the necessary corrections. Specifically, we have addressed the following issues:

In the "Conclusion" section, we have corrected the typo from "relay" to "rely" to ensure the  meaning is conveyed accurately. In Section 5.1.1, we have rectified the typo "thatelectric" to the "that electric". We have added the missing dot at the end of the first sentence of Section 4.1 to ensure proper punctuation.

Thank you for your valuable comment and for providing us with the reference to a relevant study on sparse convolution. We appreciate your suggestion and will certainly consider it for our future work.

In the revised version of the manuscript, we have discussed the recommended reference [2] and the potential incorporation of sparse convolution techniques into our research, which can be found in the last paragraph of Section 4.3.1, Page 7: 
In addition to the TCN used in our encoder, we can incorporate other convolutional frameworks into our model, such as sparse convolutions [2][28], which have shown promise in the field of 3D reconstruction. Notably, the study presented in [2] introduces the concept of sparsity-invariant convolution for handling irregularly sampled time series. This research offers valuable insights that can significantly contribute to solving the challenge of forecasting irregularly sampled time series using our proposed model.

We are particularly interested in exploring the proposed sparsity-invariant convolution from [2], as it offers valuable insights that can aid us in addressing the challenge of forecasting irregularly sampled time series. By investigating and adapting these techniques, we aim to enhance the accuracy and effectiveness of our forecasting models in such scenarios.

Furthermore, we recognize the potential of applying sparse convolution in the specific domain of 3D reconstruction. While our current work focuses on time series forecasting, we believe that exploring the application of sparse convolution in 3D reconstruction can open up new possibilities and contribute to advancements in both fields.

We sincerely appreciate your suggestion and the thoughtful review of our manuscript. Your feedback has been invaluable in improving the quality and scope of our research. 

-----End of Response to Reviewer #7------



由于给定的ETTh1数据集可能包含多个变量(每个数据点包括目标值“油温”和六个电力负荷特征)，实现单变量预测可以理解为:目标值"油温”受多个电力负荷特征变量影响，我们选取其中的一个变量(默认设置是数据的第一列，不同数据集有不同的选取方式)，模型学习该变量和目标值的对应关系。 多元时间序列预测结合多个变量来预测期望值。我们仍然以ETTh1作为例子，多变量预测可以理解为：目标值“油温”受多个变量影响，我们选取其中的多个变量(默认设置为全部六个负荷特征)，我们的模型学习这多个变量和目标值的关系。



Univariate prediction can be interpreted as follows: the target value “oil temperature” is influenced by several power load characteristic variables, and we choose one of them (the default choice is the first column of the dataset, although different datasets may have different selection methods). The model then learns the mapping between this chosen variable and the target value.
Multivariate time series forecasting involves predicting an outcome by integrating information from multiple variables. Taking ETTh1 as an example, multivariate prediction can be visualized as: the target value “oil temperature” is influenced by several variables, and we select multiple of these variables (by default, all six load characteristics). The model then discerns the relationships between these selected variables and the target value.
